One-particle irreducibility of Vilkovisky-DeWitt effective action

The effective action formalism introduced by Vilkovisky and later modified by DeWitt is completely covariant suitable for obtaining an effective action that is independent of the parametrization of the quantum fields. Among a few basic properties of an effective action, one property is that it can be written as a sum of one-particle irreducible diagrams. In this work, we verify this property up to three-loop order for Vilkovisky-Dewitt effective action (VDEA) by solving the equations satisfied by VDEA written down in the original parametrization for non-gauge theories.

==> Extra.tex <==
\nonumber\\&+
    \frac{3^4\times 3}{6^4}\begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)}]
    \begin{feynman}
    \vertex (a) at (0,0);
    \node [dot] (b) at (0.5,0);
    \node [dot] (c) at (1,0);
    \node [dot] (d) at (1.5,0);
    \vertex (e) at (0,-0.75);
    \node [dot] (f) at (0.5,-0.75);
    \node [dot] (g) at (1,-0.75);
    \node [dot] (h) at (1.5,-0.75);
    \diagram*{(a) -- [red, half right] (b) -- [red] (c) -- [red, half right] (d) -- [red, half right] (c) -- [red] (b) -- [red, half right] (a)};
    \diagram*{(e) -- [red, half right] (f) -- [red] (g) -- [red, half right] (h) -- [red, half right] (g) -- [red] (f) -- [red, half right] (e)};
    \end{feynman}
    \end{tikzpicture}+
    \frac{3^4\times 3}{6^4}\begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)}]
    \begin{feynman}
    \end{feynman}
    \end{tikzpicture}

    \rightarrow\begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)}]
    \begin{feynman}
    \vertex (a) at (0,0);
    \node [dot] (b) at (1,0);
    \vertex (c) at (1.70,0.70);
    \vertex (d) at (1.70,-0.70);
    \diagram*{(a) -- [red, quarter right] (b) -- [red, quarter right] (c) -- [red, quarter right] (b) -- [red, quarter right] (a)};
    \diagram*{(b) -- [red, quarter right] (d) -- [red, quarter right] (b)};
    \end{feynman}
    \end{tikzpicture}

==> Sec3old.tex <==
We give only a brief introduction to the Vilkovisky-DeWitt effective action in this section. Emphasis has been laid on the methods to compute VDEA following which we focus on its one-particle irreducibility. We suggest to interested readers the detailed and pedagogical review found in \cite{tomsbook} and \cite{Odintsovbook} (Chapter 6 of \cite{tomsbook} contains most of the details about things that bear only a brief mention in this paper). The Vilkovisky-DeWitt effective action is independent of the parametrization of quantum fields, unlike standard effective action \cite{unique}. The following is the integrodifferential equation for the Vilkovisky effective action for non-gauge theories;

\begin{align}\label{vdea1}
    e^{\frac{i}{\hbar}\tilde\Gamma[\bar\varphi,\varphi_*]} = \int \mathcal{D}\varphi \ \exp{\frac{i}{\hbar}\left\{S[\varphi]+\hat\Gamma_{,i}[v^i;\varphi_*]\left(v^i-\sigma^i\right)\right\}}
\end{align}
The quantities found in this equation can be explained as follows.
\begin{itemize}
    \item The field variables are denoted by $\varphi^i$ where the index $i$ is to be interpreted using DeWitt's notation. The field variables $\varphi^i$ may be considered as coordinates of a point in a Riemannian manifold. 
    \item $\sigma^i[\varphi_*, \varphi]$ is a vector at coordinate $\varphi_*$ tangent to the geodesic connecting the coordinates $\varphi^i_*$ and $\varphi^i$. The point $\varphi_*^i$ is to be considered as the origin for the normal coordinates system formed locally on the manifold. $\sigma^i[\varphi_*,\varphi]$ is crucial for the covariance of Vilkovisky's effective action formalism.
    \item $v^i = \sigma^i[\varphi_*,\bar\varphi]$, where the mean field $\bar\varphi$ is defined through the equation $\sigma^i[\varphi_*,\bar\varphi] = \langle \sigma^i[\varphi_*,\varphi]\rangle$. The angular brackets denote the average defined in the path integral formalism,
    \begin{align}
        \langle F[\varphi]\rangle = e^{-\frac{i}{\hbar}\tilde\Gamma[\bar\varphi,\varphi_*]}\int \mathcal{D}\varphi \ F[\varphi] \exp{\frac{i}{\hbar}\left\{S[\varphi]+\hat\Gamma_{,i}[v^i;\varphi_*]\left(v^i-\sigma^i\right)\right\}}
    \end{align}

    \item The Vilkovisky effective action $\Gamma$ can be regarded either as a function of the original mean fields $\bar\varphi^i$, or $v^i$, i.e. $\Gamma \equiv \tilde\Gamma[\bar\varphi,\varphi_*]\equiv\hat\Gamma[v^i,\varphi_*]$. Note that we have placed a tilde over $\Gamma$ if it is regarded as a function of the original mean fields $\bar\varphi^i$ and we have placed a hat over $\Gamma$ if it is regarded as a function of $v^i$ (This notation can be found in \cite{Rebhan:1986wp, Rebhan:1987cd}).
\end{itemize}


The variational derivative of $\hat\Gamma[v^i;\varphi_*]$ in (\ref{vdea1}) can be expressed in terms of $\tilde\Gamma[\bar\varphi,\varphi_*]$ through the use of simple chain rule giving us the following equation.

\begin{align}\label{vdea2}
    e^{\frac{i}{\hbar}\tilde\Gamma[\bar\varphi,\varphi_*]} = \int \mathcal{D}\varphi \ \exp{\frac{i}{\hbar}\left\{S[\varphi]+\tilde\Gamma_{,j}[\bar\varphi,\varphi_*]v^j{}_{,i}\left(v^i-\sigma^i\right)\right\}}
\end{align}

It was shown in \cite{Burgess:1987zi} that although $\Gamma[\bar\varphi,\varphi_*]$ in (\ref{vdea1}) depends on $\varphi_*$, any choice of $\varphi_*$ defines an equally good effective action. DeWitt \cite{Batalin:1987fw} has further shown that the choice $\varphi^i_* = \bar\varphi^i$ is easiest for the calculation of $\tilde\Gamma[\bar\varphi, \varphi_*]$. The ``Vilkovisky-DeWitt" effective action or ``VDEA" is then defined by setting $\varphi_*$ equal to $\bar\varphi$ in the Vilkovisky effective action,

\begin{align}
    \tilde\Gamma[\bar\varphi,\varphi_*]|_{\varphi_*=\bar\varphi} = \Gamma[\bar\varphi]
\end{align}

It turns out there are at least two methods to compute VDEA from either (\ref{vdea1}) or (\ref{vdea2}): 

\begin{enumerate}
    \item The first method is to solve (\ref{vdea1}) without invoking the identification $\varphi_*=\bar\varphi$ and carrying out the perturbative expansion of both sides of (\ref{vdea1})  in terms of the variable $\sigma^i$ about $\sigma^i=v^i$. The limit $\varphi_* = \bar\varphi$ is taken after computing $\hat\Gamma[v^i;\varphi_*]$

    \item The second method is to take the limit $\varphi_*=\varphi$ in (\ref{vdea2}) itself and then proceed with the perturbative expansion of both sides of (\ref{vdea2}) in terms of the variable $\sigma^i$ about $\sigma^i=0$ using the fact that $v^i=0$ when $\varphi_*=\varphi$. The variable $\sigma^i$ is then expanded in normal coordinates followed by the path integral carried out in the original parametrization $\varphi^i$.
\end{enumerate}

Let us discuss these methods briefly. The first method results in a straightforward use of (\ref{vdea1}) with the requirement of changing the path integral variable: $\varphi^i\rightarrow\sigma^i$. This introduces a Jacobian which must be taken into account while performing the perturbative expansion. For perturbative expansion, the covariant Taylor expansion of the classical action must be carried out on the R.H.S. of (\ref{vdea1}) which involves variational derivatives of the classical action $S[\bar\varphi]$ wrt. $v^i[\varphi_*,\bar\varphi]$ because we expand around $\sigma^i=v^i$;

\begin{align}\label{covtaylor}
  S[\varphi]=S[\bar\varphi] + \sum_{n=1}^\infty\frac{1}{n!}\frac{\delta^n S[\bar\varphi]}{\delta v^{i_1}\delta v^{i_2} ... \delta v^{i_n}}(\sigma^{i_1}-v^{i_1})(\sigma^{i_2}-v^{i_2})...(\sigma^{i_n}-v^{i_n}).
\end{align}

These functional derivatives appear once we have computed $\tilde\Gamma[\bar\varphi;\varphi_*]$ up to a desired order and are in general given by an infinite sum of the conventional functional derivatives;

\begin{align}\label{vder}
    \frac{\delta^n S[\bar\varphi]}{\delta v^{i_1}\delta v^{i_2} ... \delta v^{i_n}} = (-1)^nS_{;(i_1i_2...i_n)}[\bar\varphi] + \sum_{m=n+1}^\infty\frac{(-1)^m}{(m-n)!}S_{;(i_1i_2...i_m)}v^{i_{n+1}}v^{i_{n+2}}...v^{i_m},
\end{align}

    making them impossible to compute them. However when we carry out the final step of the calculation, i.e. take the limit $\varphi_*\rightarrow\bar\varphi$, we observe that the infinite sum part of (\ref{vder}) vanishes leaving behind symmetrized covariant functional derivatives of the classical action wrt. the mean fields in the original parametrization. These can be computed as usual for any theory using the field space connections.

The second method can be used after we rewrite $(\ref{vdea2})$ completely in terms of $\varphi$ and $\bar\varphi$ by taking the limit $\varphi_*=\varphi$. This requires us to compute the following limit in (\ref{vdea2}),

\begin{align}
    \frac{\delta\tilde\Gamma[\bar\varphi,\varphi_*]}{\delta \bar\varphi^j}\Big|_{\varphi_*=\bar\varphi}
\end{align}
This is not simply $\frac{\Gamma[\bar\varphi]}{\delta \bar\varphi^j}$ because the derivative must be computed before taking the limit inside $\Gamma[\bar\varphi,\varphi_*]$. To calculate the limit properly we require the following identity which can be derived from (\ref{vdea2})

\begin{align}\label{3id1}
    \frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta \varphi^i_*} = \frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta \bar\varphi^j}(v^j{}_{;i}-C^j{}_{i}[\bar\varphi]),
\end{align}
where 
\begin{align}
    C^i{}_{j}[\bar\varphi]=\langle\sigma^j{}_{;i}[\bar\varphi,\varphi]\rangle.
\end{align}
After taking the limit $\varphi_*=\bar\varphi$ in (\ref{3id1}) we obtain the following identity using (\ref{2id1}),

\begin{align}\label{3id2}
    \frac{\delta\tilde\Gamma[\bar\varphi,\varphi_*]}{\delta \bar\varphi^i}\Big|_{\varphi_*=\bar\varphi} = C^{-1i}{}_{j}[\bar\varphi]\times\lim_{\varphi_*\rightarrow\bar\varphi}\left(\frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta\varphi_*^j}+\frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta\bar\varphi^j}\right)
\end{align}

Finally, we note that
\begin{align}
    \delta\Gamma[\bar\varphi]
    &=\lim_{\varphi_*=\bar\varphi}\delta\tilde\Gamma[\varphi_*;\varphi]\nonumber\\
    &=\lim_{\varphi_*=\bar\varphi}\left(\frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta\varphi_*^i}\delta\varphi_*^i+\frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta\bar\varphi^i}\delta\bar\varphi^i\right)\nonumber\\
    &=\lim_{\varphi_*=\bar\varphi}\left(\frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta\varphi_*^i}+\frac{\delta\tilde\Gamma[\bar\varphi;\varphi_*]}{\delta\bar\varphi^i}\right)\delta\bar\varphi^i\label{3id3}
\end{align}
Using (\ref{3id3}) in (\ref{3id2}) we find,

\begin{align}
    \frac{\delta\tilde\Gamma[\bar\varphi,\varphi_*]}{\delta \bar\varphi^i}\Big|_{\varphi_*=\bar\varphi} = C^{-1i}{}_{j}[\bar\varphi]\frac{\delta\Gamma[\bar\varphi]}{\delta\bar\varphi^j}
\end{align}
Now we can rewrite (\ref{vdea2}) as follows,

\begin{align}\label{vdea2re}
    e^{\frac{i}{\hbar}\Gamma[\bar\varphi]} = \int \mathcal{D}\varphi \ \exp{\frac{i}{\hbar}\left\{S[\varphi]-\sigma^i[\bar\varphi,\varphi]C^{-1j}{}_{,i}[\bar\varphi]\Gamma_{,j}[\bar\varphi]\right\}}
\end{align}
This equation for $\Gamma[\bar\varphi]$ is supplemented by an equation for $C^i{}_j[\bar\varphi]$

\begin{align}\label{Ceq}
    C^i{}_j[\bar\varphi]=e^{-\frac{i}{\hbar}\Gamma[\bar\varphi]}\int \mathcal{D}\varphi \ \sigma^i{}_{;j}[\bar\varphi,\varphi]\exp{\frac{i}{\hbar}\left\{S[\varphi]-\sigma^i[\bar\varphi,\varphi]C^{-1j}{}_{,i}[\bar\varphi]\Gamma_{,j}[\bar\varphi]\right\}}
\end{align}
(\ref{vdea2re}) and (\ref{Ceq}) thus form a set of coupled integro-differential equations for $\Gamma[\bar\varphi]$ and $C^i{}_j[\bar\varphi]$. The computation of the VDEA then involves solving both (\ref{vdea2re}) and (\ref{Ceq}) simultaneously up to any desired order. Since the limit $\varphi_* = \bar\varphi$ has already been taken in (\ref{vdea2re}) and (\ref{Ceq}) we just need to use the covariant Taylor series expansion about $\sigma^i=0$ with all the vertices being the conventional ones, i.e. $S_{;(i_1i_2...i_n)}$. 

Let us discuss the merits and demerits of using either of these methods. We observe that method (1) is relatively simple since we need to solve only one equation whereas method (2) involves coupled integro-differential equations which are much more complicated and tedious to solve as we will see when we use it to show whether VDEA consists of 1PI diagrams or not. The only problem with method (1) is that the change in the variable of the path integral introduces a jacobian which as shown in \cite{Rebhan:1987cd} starts to contribute from two-loop order onwards. As usual, the jacobian can be dealt with easily by introducing the usual Fadeev-Popov ghosts in the path integral as shown in \cite{Rebhan:1987cd}. The only merit of method (2) is that it allows us to carry out the perturbative expansion in the original parametrization starting from (\ref{vdea2re}) which involves only conventional vertices from the beginning. This however, does not seem at all to be an advantage over method (1) since although method (1) involves at an intermediate step an infinite sum of vertices finally it is the conventional vertices that are to be computed which can be done easily for any interacting theory. The result of this discussion is that method (1) is more of a practical use for computing VDEA. It is simple to show that VDEA is a sum of one-particle irreducible diagrams through the use of method (1) \cite{tomsbook, Rebhan:1987cd}. For consistency, it becomes imperative to show that this holds even if one chooses to use method (2) which is what forms the main motive of this paper. We also note that up to one-loop order there is no difference between the two methods discussed since $C^{-1i}{}_{j}[\bar\varphi]$ only makes non-trivial contributions when VDEA is computed beyond one-loop (See \ref{SecIV}). \textcolor{red}{cite}. In the next section, we perturbatively expand VDEA in integral powers of $\hbar$.

==> Section2.tex <==



\begin{align}\label{2id1}
    v^i{}_{;j}[\varphi_*,\bar\varphi]|_{\varphi_*=\bar\varphi} = \delta^i{}_{j}
\end{align}

\begin{align}\label{covtaylor}
    S[\varphi]=S[\bar\varphi] + \sum_{n=1}^\infty\frac{1}{n!}\frac{\delta^n S[\bar\varphi]}{\delta v^{i_1}\delta v^{i_2} ... \delta v^{i_n}}(\sigma^{i_1}-v^{i_1})(\sigma^{i_2}-v^{i_2})...(\sigma^{i_n}-v^{i_n})
\end{align}


\begin{align}\label{vder}
    \frac{\delta^n S[\bar\varphi]}{\delta v^{i_1}\delta v^{i_2} ... \delta v^{i_n}} = (-1)^nS_{;(i_1i_2...i_n)}[\bar\varphi] + \sum_{m=n+1}^\infty\frac{(-1)^m}{(m-n)!}S_{;(i_1i_2...i_m)}v^{i_{n+1}}v^{i_{n+2}}...v^{i_m}
\end{align}

\begin{align}
    \sigma^i[\bar\varphi,\varphi]=-\eta^i + \sum_{n=1}^\infty\sigma^i_{(n)}
\end{align}
where $\eta^i = \varphi^i-\bar\varphi^i$
